Enhancing Logical Reasoning in Large Language Models through Graph-based Synthetic Data

Despite recent advances in training and prompting strategies for Large Language Models (LLMs), these models continue to face challenges with complex logical reasoning tasks that involve long reasoning chains. In this work, we explore the potential and limitations of using graph-based synthetic reasoning data as training signals to enhance LLMs' reasoning capabilities. Our extensive experiments, conducted on two established natural language reasoning tasks -- inductive reasoning and spatial reasoning -- demonstrate that supervised fine-tuning (SFT) with synthetic graph-based reasoning data effectively enhances LLMs' reasoning performance without compromising their effectiveness on other standard evaluation benchmarks.

==> section/related_work.tex <==
\section{Related Works}
%  across diverse reasoning tasks.
% Reasoning Capabilities of Large Language Models (LLMs) have 
% Large Language Models (LLMs)~\cite{} have demonstrated notable reasoning capabilities, sparking research into methods for improvement~\cite{} and evaluation~\cite{}.

\paragraph{Logical Reasoning:}
Logical reasoning has been highlighted in language modeling~\cite{zhang2023improved, yang2024large, li2024improving}. 
Especially, \citet{yang2024large} reveal that LLMs possess the capability of latent multi-hop reasoning, in which,
however, the moderative evidence of second-hop reasoning 
does not become stronger with increasing model size.







\paragraph{Reasoning Datasets:}
Various question-and-answer (QA) datasets have been proposed to evaluate the logical reasoning ability of language models.
Commonly used datasets include
HotpotQA~\cite{yang2018hotpotqa}, 
ComplexWebQuestions~\cite{talmor2018web},
QAngaroo~\cite{welbl2018constructing} and CLUTTER~\cite{sinha2019clutrr}.
These datasets emphasize the knowledge-based reasoning ability of language models. 
Besides, several datasets focus on spatial reasoning, e.g., 
bAbI~\cite{weston2015AICompleteQuestionAnswering},
SpartQA~\cite{mirzaee2021SPARTQATextualQuestion} and StepGame~\cite{shi2022StepGameNewBenchmark}.











\paragraph{Synthetic datasets:} A new trend in probing various LLMs capabilities, especially in the case of reasoning, is through synthetic data that allows for a more systematic evaluation. Previous work has developed synthetic datasets for probing and improving various kinds of reasoning including logical reasoning \cite{tafjord2021ProofWriterGeneratingImplications,kazemi2023BoardgameQADatasetNatural,saparov2023TestingGeneralDeductive}, mathematical reasoning \cite{srivastava2024FunctionalBenchmarksRobust} \cite{kazemi2023GeomVerseSystematicEvaluation} and temporal reasoning \cite{fatemi2024TestTimeBenchmark}. Several works add KG triplet information directly to the LM input \cite{agarwal2021KnowledgeGraphBased}.

% yuan2024advancing: fine-tune llm for logical reasoning improvmeent
